Bringing Cognitive Augmentation to Web Browsing Accessibility

In this paper we explore the opportunities brought by cognitive augmentation to provide a more natural and accessible web browsing experience. We explore these opportunities through \textit{conversational web browsing}, an emerging interaction paradigm for the Web that enables blind and visually impaired users (BVIP), as well as regular users, to access the contents and features of websites through conversational agents. Informed by the literature, our previous work and prototyping exercises, we derive a conceptual framework for supporting BVIP conversational web browsing needs, to then focus on the challenges of automatically providing this support, describing our early work and prototype that leverage heuristics that consider structural and content features only.

==> sections/background.tex <==
An approach to providing conversational access to artefacts is to enable developers and content producers to provide appropriate annotations [xx].
%idea
Early approaches can be traced back to enabling access to web pages through telephone call services. The idea was to provide voice-based access by either developing web pages using standards such as VoiceXML \cite{oshry2007voice}, or applying \textit{transcoding} on websites to convert HTML code into VoiceXML code\cite{shao2002annotations}. Since the focus was to enable access from telephones, and not actually engaging in a conversation with users, the type of experience provided is closer to that of screen reading than to modern conversational agents. %Yet, the concept of providing external annotations to guide the transcoding process emerged in this space, so as to allow developers to decide what features and content to expose and how \cite{shao2002annotations}.
%
Another general approach to voice-based accessible information is to rely on accessibility technical specifications, such as Accessible Rich Internet Applications (WAI-ARIA) \cite{diggs2016accessible}. Based on annotations provided by such specifications, screen readers are able to read out and navigate documents, and in recent works, to even accept basic voice commands \cite{ashok2015capti}.
The challenge in this regard is the adoption of accessibility annotations by developers and content producers.
%
A recent report analysing 1 Million websites \cite{webaim2019million} pointed to staggering 97.8\% of websites with detectable accessibility errors, illustrating the extent of adoption on the Web.

Collaborative metadata augmentation approaches  \cite{bigham2007accessmonkey,takagi2008social} instead rely on the crowd to "fix" accessibility problems or provide annotations for voice-based access. The Social Accessibility project \cite{sato2010exploratory} is one of these initiatives whose database supports various non visual browsers. 
Ripa et al. \cite{ripa2019end} focus on making informational queries over content intensive websites accessible via voice-based interfaces (e.g., smart speakers), relying on augmentations provided and shared by end-users. 
%challenge?
% the rate of new content and services on the web
% significant community to make it viable
% what about other type of artefacts?

Automatic approaches 
page segmentation \cite{cormier2016purely}
discovering the accessibility roles \cite{akpinar2017discovering}
detecting transactions \cite{islam2010improving}
predicting next actions \cite{puzis2013predictive}




